End-to-End Learning of Representations for Asynchronous Event-Based Data

Event cameras are vision sensors that record asynchronous streams of per-pixel brightness changes, referred to as "events". They have appealing advantages over frame-based cameras for computer vision, including high temporal resolution, high dynamic range, and no motion blur. Due to the sparse, non-uniform spatiotemporal layout of the event signal, pattern recognition algorithms typically aggregate events into a grid-based representation and subsequently process it by a standard vision pipeline, e.g., Convolutional Neural Network (CNN). In this work, we introduce a general framework to convert event streams into grid-based representations through a sequence of differentiable operations. Our framework comes with two main advantages: (i) allows learning the input event representation together with the task dedicated network in an end to end manner, and (ii) lays out a taxonomy that unifies the majority of extant event representations in the literature and identifies novel ones. Empirically, we show that our approach to learning the event representation end-to-end yields an improvement of approximately 12% on optical flow estimation and object recognition over state-of-the-art methods.

==> images_tex/optic_flow_image.tex <==
\begin{figure*}
    \centering
    \begin{tabular}{ccc}
    	\emph{indoor\_flying1}&\emph{indoor\_flying2}&\emph{indoor\_flying3}]\\ 

    	\includegraphics[height=2.7in]{images/optic_flow_indoor1.png}&
    	\includegraphics[height=2.7in]{images/optic_flow_indoor2.png}&
    	\includegraphics[height=2.7in]{images/optic_flow_indoor3.png}\\
    	(a)&(b)&(c)\\
    \end{tabular}
    \caption{Visualization of the flow predicted by our network on the MVSEC datasets: (a) \emph{indoor\_flying1}, (b) \emph{indoor\_flying2}, and (c) \emph{indoor\_flying3}.
    The top row shows ground truth optical flow and the bottom shows the prediction from our network.
    As the event signal only provides sparse information, we show the flow only where events are triggered.}
    \label{fig:qualitative_flow}
\end{figure*}

==> images_tex/optic_flow_sota.tex <==
\begin{table*}[]
\begin{tabular}{c|c|ccc|c|cc}
\hline
\multirow{2}{*}{Representation} & \multirow{2}{*}{Reference} & \multicolumn{2}{c}{indoor\_flying1}                            & \multicolumn{2}{c|}{indoor\_flying2} & \multicolumn{2}{c}{indoor\_flying3}       \\ \cline{3-8}  
&                                                            & \multicolumn{1}{c|}{AEE}  & \multicolumn{1}{c|}{\% Outlier}    & AEE                     & \% Outlier & \multicolumn{1}{c|}{AEE} & \% Outlier\\\hline
EST (learnt)                    & ours                       & \multicolumn{1}{c|}{0.97} & \multicolumn{1}{c|}{\textbf{0.91}} & \textbf{1.38}        & \textbf{6.47} & \multicolumn{1}{c|}{1.43} & \textbf{8.20} \\
EST (exponential)               & ours                       & \multicolumn{1}{c|}{\textbf{0.96}} & \multicolumn{1}{c|}{1.27} & 1.58                 & 10.5          & \multicolumn{1}{c|}{\textbf{1.40}} & 9.44 \\
EV-FlowNet                      & \cite{Zhu18rss}            & \multicolumn{1}{c|}{1.03} & \multicolumn{1}{c|}{2.2}           & 1.72                 & 15.1          & \multicolumn{1}{c|}{1.53}          & 11.9 \\
Voxel Grid                      & \cite{Zhu19cvpr}          & \multicolumn{1}{c|}{\textbf{0.96}} & \multicolumn{1}{c|}{1.47}          & 1.65                 & 14.6          & \multicolumn{1}{c|}{1.45}          & 11.4 \\
2 Channel Image                 & \cite{Maqueda18cvpr}       & \multicolumn{1}{c|}{1.21} & \multicolumn{1}{c|}{4.49}          & \multicolumn{1}{c|}{2.03} & 22.8     & \multicolumn{1}{c|}{1.84}          & 17.7 \\\hline
\end{tabular}
\caption{}
\label{tab:optic_flow_sota}
\end{table*}
